Censored Quantile Regression Forest

Random forests are powerful non-parametric regression method but are severely limited in their usage in the presence of randomly censored observations, and naively applied can exhibit poor predictive performance due to the incurred biases. Based on a local adaptive representation of random forests, we develop its regression adjustment for randomly censored regression quantile models. Regression adjustment is based on a new estimating equation that adapts to censoring and leads to quantile score whenever the data do not exhibit censoring. The proposed procedure named {\it censored quantile regression forest}, allows us to estimate quantiles of time-to-event without any parametric modeling assumption. We establish its consistency under mild model specifications. Numerical studies showcase a clear advantage of the proposed procedure.

==> related_work.tex <==
\section{Related Work}

In the case of right censoring, most non-parametric recursive partitioning algorithms in the existing literature rely on survival tree or its ensembles. \cite{ishwaran2008random} proposed random survival forest (RSF) algorithm in which each tree is built by maximizing the between-node log-rank statistic. However, it is not directly estimating the conditional quantiles but instead estimating the cumulative hazard. \cite{zhu2012recursively} proposed the recursively imputed survival trees (RIST) algorithm with the same splitting criterion for each individual tree but different ensemble scheme. Other similar methods relying on different kinds of survival trees were proposed in \cite{gordon1985tree}, \cite{segal1988regression}, \cite{davis1989exponential}, \cite{leblanc1992relative}, and \cite{leblanc1993survival}. All these methods as mentioned above use splitting rules specifically designed to deal with the right censored data. Despite different splitting strategies, they all rely on the proportional hazard assumption and cannot reduce to a loss-based method that might ordinarily be used in the situation with no censoring.

\cite{molinaro2004tree} proposed a tree method based on the inverse probability censoring \citep{robins1994estimation} weighted (IPCW) loss function which reduces to the full data loss function used by CART in the absence of censoring. \cite{hothorn2005survival} then extended the IPCW idea and proposed a forest-type method in which each tree is trained on resampled observations according to inverse probability censoring weights. However, the censored data always get weights zero and hence only uncensored observations will be resampled. As pointed out by \cite{robins1994estimation}, the inverse probability weighted estimators are inefficient because of their failure to utilize all the information available on observations with missing or partially missing data. 
